From point forecasts to multivariate probabilistic forecasts: The Schaake shuffle for day-ahead electricity price forecasting

Modeling price risks is crucial for economic decision making in energy markets. Besides the risk of a single price, the dependence structure of multiple prices is often relevant. We therefore propose a generic and easy-to-implement method for creating multivariate probabilistic forecasts based on univariate point forecasts of day-ahead electricity prices. While each univariate point forecast refers to one of the day's 24 hours, the multivariate forecast distribution models dependencies across hours. The proposed method is based on simple copula techniques and an optional time series component. We illustrate the method for five benchmark data sets recently provided by Lago et al. (2020). Furthermore, we demonstrate an example for constructing realistic prediction intervals for the weighted sum of consecutive electricity prices, as, e.g., needed for pricing individual load profiles.

==> Energy ECC - arxiv/table_AR.tex <==
%% Standardisation done with parameters of one TS! Raw-Standardized uses var/bias of last 90 days%%%%%%%%%%%%%%

\begin{table}[ht]
\centering
\begin{tabular}{@{\extracolsep{4pt}}lrrrr@{}}

\hline
Setting& Energy Score& CRPS&\multicolumn{2}{c}{$p$-values}\\
&&&(a)&(b)\\
\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-5} 

\\[-0.95em]
 EPEX-DE \\
\hline
Schaake-NP  &  19.837&  3.297& & \\
Schaake-P  &  21.138&  3.611& $<$0.001 &$<$0.001\\
Schaake-Raw  &  19.787& 3.266& 0.685 &0.133\\
I-NP  &  20.398& 3.297& $<$0.001& \\
I-P  &  21.452& 3.611& $<$0.001 &$<$0.001\\
I-Raw  &  20.322& 3.266& $<$0.001& 0.133\\
\hline
%%%%%%%%%%%%%%%%%
\\[-0.95em]
\multicolumn{4}{@{}l}{Pennsylvania-New Jersey-Maryland (PJM) }\\ \hline    
Schaake-NP  &  14.594&  2.394& & \\
Schaake-P  &  15.318&  2.581& $<$0.001 &$<$0.001\\
Schaake-Raw  &  14.791& 2.436& 0.162 &0.047\\
I-NP  &  15.133& 2.394& $<$0.001& \\
I-P  &  15.687& 2.581& $<$0.001 &$<$0.001\\
I-Raw  &  15.426& 2.436& $<$0.001& 0.047\\
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.95em]

EPEX-BE   \\
\hline  
Schaake-NP  &  35.13&  5.503& & \\
Schaake-P  &  38.64&  6.134& $<$0.001 &$<$0.001\\
Schaake-Raw  &  33.488& 5.311& 0.012 &0.001\\
I-NP  &  36.423& 5.503& $<$0.001& \\
I-P  &  38.868& 6.134& $<$0.001 &$<$0.001\\
I-Raw  &  34.642& 5.311& 0.444& 0.001\\

\hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.95em]
EPEX-FR \\
\hline 
Schaake-NP  &  22.553&  3.307& & \\
Schaake-P  &  23.578&  3.515& 0.001 &$<$0.001\\
Schaake-Raw  &  21.203& 3.243& 0.097 &0.119\\
I-NP  &  23.088& 3.307& $<$0.001& \\
I-P  &  23.935& 3.515& $<$0.001 &$<$0.001\\
I-Raw  &  21.633& 3.243& 0.259& 0.119\\
\hline 


%%%%%%%%%%%%%%%%%%%%%%%
\\[-0.95em]
Nord Pole  \\
\hline
Schaake-NP  &  9.729&  1.571& & \\
Schaake-P  &  10.437&  1.72& $<$0.001 &$<$0.001\\
Schaake-Raw  &  9.904& 1.626& 0.007 &$<$0.001\\
I-NP  &  10.179& 1.571& $<$0.001& \\
I-P  &  10.657& 1.72& $<$0.001 &$<$0.001\\
I-Raw  &  10.189& 1.626& $<$0.001& $<$0.001\\


\hline



\end{tabular}
\caption{Energy Score and CRPS for several variants of proposed method and five benchmark data sets. (a) $p$-value of Diebold-Mariano tests for equal Energy Score, compared to Schaake-NP. (b) $p$-value of Diebold-Mariano tests for equal CRPS, compared to Schaake-NP. Blank cells indicate that scores are equal by construction, so that the test is undefined.}

\label{tabres}
\end{table}


